JWST's PEARLS: Prime Extragalactic Areas for Reionization and Lensing Science: Project Overview and First Results

We give an overview and describe the rationale, methods, and first results from NIRCam images of the JWST "Prime Extragalactic Areas for Reionization and Lensing Science" ("PEARLS") project. PEARLS uses up to eight NIRCam filters to survey several prime extragalactic survey areas: two fields at the North Ecliptic Pole (NEP); seven gravitationally lensing clusters; two high redshift proto-clusters; and the iconic backlit VV 191 galaxy system to map its dust attenuation. PEARLS also includes NIRISS spectra for one of the NEP fields and NIRSpec spectra of two high-redshift quasars. The main goal of PEARLS is to study the epoch of galaxy assembly, AGN growth, and First Light. Five fields, the JWST NEP Time-Domain Field (TDF), IRAC Dark Field (IDF), and three lensing clusters, will be observed in up to four epochs over a year. The cadence and sensitivity of the imaging data are ideally suited to find faint variable objects such as weak AGN, high-redshift supernovae, and cluster caustic transits. Both NEP fields have sightlines through our Galaxy, providing significant numbers of very faint brown dwarfs whose proper motions can be studied. Observations from the first spoke in the NEP TDF are public. This paper presents our first PEARLS observations, their NIRCam data reduction and analysis, our first object catalogs, the 0.9-4.5 $\mu$m galaxy counts and Integrated Galaxy Light. We assess the JWST sky brightness in 13 NIRCam filters, yielding our first constraints to diffuse light at 0.9-4.5 {\mu}m. PEARLS is designed to be of lasting benefit to the community.

==> RUN <==
#!/bin/sh
#
# pdflatex will include PDF figure files:  fig*.pdf. Run as:
# > pdflltxg*
#
# pdflltxg* doesn't always work on linux or Mac, since it assumes that
# the bib file ends with .bib e.g.: references_v7.bib
#
# May need to crop empty space from all fig*.pdf files first by using:
# > pdfcrop fig1.pdf 
# > mv fig1-crop.pdf fig1.pdf
# 
# Or convert directly from .ps to .pdf without generating additional white space: 
# ps2pdf -dEPSCrop fig1.ps

pdflatex        windhorst_pearls_overview_v5.latex

bibtex          windhorst_pearls_overview_v5
bibtex          references_pearls_overview

pdflatex        windhorst_pearls_overview_v5.latex

pdflatex        windhorst_pearls_overview_v5.latex

### dvips       windhorst_pearls_overview_v5.dvi -o windhorst_pearls_overview_v5.ps

### ps2pdf14    windhorst_pearls_overview_v5.ps  -o windhorst_pearls_overview_v5.pdf


acroread   windhorst_pearls_overview_v5.pdf & #### 

#### open -a preview windhorst_pearls_overview_v5.pdf & #### 


\rm             *.aux *.log *.out #### *Notes.bib *.bib ### *.dvi ### 


exit

